Online Censoring-Based Widely Linear Total Least lncosh Method for Improved Power System Frequency Estimation

Recently, under the presumption of a noise-free input, the augmented complex least lncosh (ACLlncosh) method was introduced for a power system frequency estimate and showed robust performance when impulsive noise polluted the output signal. However, in practical terms, noise often contaminates input signals, which drastically reduces the efficiency of the ACLlncosh method. To enhance robustness against noisy input-output while maintaining resilience to impulsive noise in the output signal, this paper proposed an online censoring-based widely linear total least lncosh (OC-WL-TLlnC) method. This method improves performance under both balanced and unbalanced settings by filtering out less valuable data via online censoring, hence reducing the computing burden. Furthermore, a variable parameter approach is incorporated to accelerate convergence and improve steady-state accuracy, thereby ensuring adaptability to dynamic power system conditions. The proposed methods significantly enhance frequency estimate performance by addressing the constraints of current techniques and offering a computationally efficient, noise-resilient solution for real-time power system monitoring.

==> sections/discussion.tex <==
\section{Discussion}\label{sec:discussion}


==> sections/myacronyms.tex <==
%! Author = federico
%! Date = 10/06/2020


\renewcommand{\baselinestretch}{0.75}\normalsize
\renewcommand{\aclabelfont}[1]{\textsc{\acsfont{#1}}}
\begin{acronym}[longest]

    \acro{t-db}[$t_{db}$]{Manuscript; This research received partial support from the National Natural Science Foundation of China under grants 62171388, 61871461, and 61571374. Haiquan Zhao,  Kaleab Derbew  are with the school of Electrical Engineering, Southwest Jiaotong University, Chengdu
	610031, China (e-mail: hqzhao\_swjtu@126.com; bekalu.derbew@gmail.com}
    \acro{t-wb}[$t_{wb}$]{wet-bulb air temperature\acroextra{, $^{\circ}$C}}
    \acro{ti}[$t_{i}$]{indoor air temperature\acroextra{, $^{\circ}$C}}
    \acro{tout}[$t_{out}$]{outdoor air temperature\acroextra{, $^{\circ}$C}}
    \acro{t-op}[$t_{o}$]{operative air temperature\acroextra{, $^{\circ}$C}}
    \acro{t-cl}[$t_{cl}$]{clothing temperature\acroextra{, $^{\circ}$C}}
    \acro{tg}[$t_{g}$]{globe temperature\acroextra{, $^{\circ}$C}}
    \acro{rh}[$RH$]{relative humidity\acroextra{, \%}}
    \acro{v}[$V$]{average air speed\acroextra{, m/s}}
    \acro{t-r}[$\overline{t_{r}}$]{mean radiant temperature\acroextra{, $^{\circ}$C}}
    \acro{clo}[$I_{cl}$]{total clothing insulation\acroextra{, clo}}
    \acro{i-cl}[$i_{cl}$]{permeation efficiency of water vapor through the clothing layer}
    \acro{met}[$M$]{rate of metabolic heat production\acroextra{, W/m\textsuperscript{2}}}
    \acro{work}[$W$]{rate of mechanical work accomplished\acroextra{, W/m\textsuperscript{2}}}
    \acro{t-sk}[$t_{sk}$]{skin mean temperature\acroextra{, $^{\circ}$C}}
    \acro{t-sk-n}[$t_{sk,n}$]{neutral skin mean temperature\acroextra{, $^{\circ}$C}}
    \acro{t-cr}[$t_{cr}$]{core mean temperature\acroextra{, $^{\circ}$C}}
    \acro{t-re}[$t_{re}$]{rectal temperature\acroextra{, $^{\circ}$C}}
    \acro{t-cr-n}[$t_{cr,n}$]{neutral core mean temperature\acroextra{, $^{\circ}$C}}
    \acro{r-cl}[$R_{cl}$]{thermal resistance of clothing\acroextra{, m\textsuperscript{2}K/W}}
    \acro{r-e-cl}[$R_{e,cl}$]{evaporative heat transfer resistance of clothing layer\acroextra{, m\textsuperscript{2}kPa/W}}
    \acro{f-cl}[$f_{cl}$]{clothing area factor $A_{cl}/A_{body}$\acroextra{, m\textsuperscript{2}K/W}}
    \acro{h}[$h$]{sum of convective $h_{c}$ and radiative $h_{r}$ heat transfer coefficients\acroextra{, W/(m\textsuperscript{2}K)}}
    \acro{h-r}[$h_{r}$]{linear radiative heat transfer coefficient\acroextra{, W/(m\textsuperscript{2}K)}}
    \acro{h-c}[$h_{c}$]{convective heat transfer coefficient\acroextra{, W/(m\textsuperscript{2}K)}}
    \acro{h-e}[$h_{e}$]{evaporative heat transfer coefficient\acroextra{, W/(m\textsuperscript{2}kPa)}}
    \acro{a}[$\alpha$]{fraction of the total body mass considered
to be thermally in the skin compartment}

    \acro{cl-a}[$A_{cl}$]{clothing surface area\acroextra{, m\textsuperscript{2}}}

    \acro{e}[$\varepsilon$]{average emissivity of clothing or body surface}
    \acro{sigma}[$\sigma$]{Stefan-Boltzmann constant\acroextra{, 5.67 x 10\textsuperscript{-8} W/(m\textsuperscript{2}K\textsuperscript{2})}}

    \acro{a-r}[$A_{r}$]{effective  radiation  area  of  the  body\acroextra{, m\textsuperscript{2}}}
    \acro{body-a}[$A_{body}$]{body surface area\acroextra{, m\textsuperscript{2}}}
    \acro{body-w}[$mass$]{body mass\acroextra{, kg}}
    \acro{body-h}[$height$]{body height\acroextra{, m}}

    \acro{pmv}[PMV]{Predicted Mean Vote}
    \acro{ppd}[PPD]{Predicted Percentage of Dissatisfied\acroextra{, \%}}
    \acro{set}[SET]{Standard Effective Temperature\acroextra{, $^{\circ}$C}}
    \acro{ce}[CE]{Cooling Effect\acroextra{, $^{\circ}$C}}
    \acro{phs}[PHS]{Predicted Heat Strain}

    \acro{BMS}[BMS]{Building Management System}
    \acro{HVAC}[HVAC]{Heating, Ventilation, and Air Conditioning}
    \acro{VAV}[VAV]{Variable Air Volume}
    \acro{AHU}[AHU]{Air Handling Unit}

    \acro{ema}[EMA]{Ecological Momentary Assessment}
    \acro{sdk}[SDK]{Software Development Kit}
    \acro{api}[API]{Application Programming Interface}

    \acro{s-cr}[$S_{cr}$]{rate of heat storage in the core compartment\acroextra{, W/m\textsuperscript{2}}}
    \acro{s-sk}[$S_{sk}$]{rate of heat storage in the skin compartment\acroextra{, W/m\textsuperscript{2}}}
    \acro{s}[$S$]{rate of heat storage in the human body\acroextra{, W/m\textsuperscript{2}}}
    \acro{e-res}[$E_{res}$]{rate of evaporative heat loss from respiration\acroextra{, W/m\textsuperscript{2}}}
    \acro{e-dif}[$E_{dif}$]{rate of evaporative heat loss from moisture diffused through the skin\acroextra{, W/m\textsuperscript{2}}}
    \acro{e-rsw}[$E_{rsw}$]{rate of evaporative heat loss from sweat evaporation\acroextra{, W/m\textsuperscript{2}}}
    \acro{e-sk}[$E_{sk}$]{total rate of evaporative heat loss from skin\acroextra{, W/m\textsuperscript{2}}}
    \acro{e-max}[$E_{max}$]{maximum rate of evaporative heat loss from skin\acroextra{, W/m\textsuperscript{2}}}
    \acro{c-res}[$C_{res}$]{rate of convective heat loss from respiration\acroextra{, W/m\textsuperscript{2}}}
    \acro{c-r}[$C + R$]{sensible heat loss from skin\acroextra{, W/m\textsuperscript{2}}}
    \acro{q-res}[$q_{res}$]{total rate of heat loss through respiration\acroextra{, W/m\textsuperscript{2}}}
    \acro{q-sk}[$q_{sk}$]{total rate of heat loss from skin\acroextra{, W/m\textsuperscript{2}}}
    \acro{w}[$w$]{skin wettedness}
    \acro{w-max}[$w_{max}$]{skin wettedness practical upper limit}
    \acro{m-sweat}[$m_{rsw}$]{rate at which regulatory sweat is generated\acroextra{, mL/h\textsuperscript{2}}}
    \acro{m-bl}[$m_{bl}$]{skin blood flow\acroextra{, L/(hm\textsuperscript{2})}}
    \acro{c-sw}[$c_{sw}$]{driving coefficient for regulatory sweating\acroextra{, g/(hKm\textsuperscript{2})}}

    \acro{p-sk}[$p_{sk,s}$]{water vapor pressure at skin\acroextra{, kPa}}
    \acro{p-a}[$p_{a}$]{water vapor pressure in ambient air\acroextra{, kPa}}

    \acro{wmo}[WMO]{World Meteorological Organization}
    \acro{who}[WHO]{World Health Organization}
    \acro{cdc}[CDC]{Centers for Disease Control and Prevention}
    \acro{noaa}[NOAA]{National Oceanic and Atmospheric Administration}
    \acro{epa}[EPA]{United States Environmental Protection Agency}
    \acro{iea}[IEA]{International Energy Agency}
    \acro{un}[UN]{United Nations}

\end{acronym}
\renewcommand{\baselinestretch}{1}\normalsize


==> sections/myglossary.tex <==
\usepackage[nonumberlist,nogroupskip]{glossaries}

\newglossaryentry{7730}
{
name={ISO~7730:2005},
description={ISO~7730:2005 is a thermal comfort standard developed by ISO}
}

\newglossaryentry{55}
{
name={ASHRAE~55--2020},
description={ASHRAE~55--2020 is a thermal comfort standard developed by ANSI and ASHRAE}
}

\makenoidxglossaries

